Formation of local and global currents in a toroidal Bose--Einstein condensate via an inhomogeneous artificial gauge field

We study the effects of a position-dependent artificial gauge field on an atomic Bose--Einstein condensate in quasi-one-dimensional and two-dimensional ring settings. The inhomogeneous artificial gauge field can induce global and local currents in the Bose--Einstein condensate via phase gradients along the ring and vortices, respectively. We observe two different regimes in the system depending on the radial size of the ring and strength of the gauge field. For weak artificial gauge fields, the angular momentum increases, as expected, in a quantized manner; however, for stronger values of the fields, the angular momentum exhibits a linear (non-quantized) behavior. We also characterize the angular momentum for non-cylindrically symmetric traps.

==> bib.tex <==
@article{Sahar_2BEC,
  title = {Symmetry breaking in binary Bose-Einstein condensates in the presence of an inhomogeneous artificial gauge field},
  author = {Hejazi, S. Sahar S. and Polo, Juan and Sachdeva, Rashi and Busch, Thomas},
  journal = {Phys. Rev. A},
  volume = {102},
  issue = {5},
  pages = {053309},
  numpages = {8},
  year = {2020},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.102.053309}
}

@article{mathey2016realizing,
	doi = {10.1088/1367-2630/18/5/055016},
	year = 2016,
	month = {may},
	publisher = {{IOP} Publishing},
	journal={New Journal of Physics},
	volume = {18},
	number = {5},
	pages = {055016},
	author = {Amy C Mathey and L Mathey},
	title = {Realizing and optimizing an atomtronic {SQUID}}
}

@article{piazza2009vortex,
  title = {Vortex-induced phase-slip dissipation in a toroidal Bose-Einstein condensate flowing through a barrier},
  author = {Piazza, F. and Collins, L. A. and Smerzi, A.},
  journal = {Phys. Rev. A},
  volume = {80},
  issue = {2},
  pages = {021601},
  numpages = {4},
  year = {2009},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.80.021601}
}


@article{dobrek1999optical,
  title = {Optical generation of vortices in trapped Bose-Einstein condensates},
  author = {Dobrek, \L{}. and Gajda, M. and Lewenstein, M. and Sengstock, K. and Birkl, G. and Ertmer, W.},
  journal = {Phys. Rev. A},
  volume = {60},
  issue = {5},
  pages = {R3381--R3384},
  numpages = {0},
  year = {1999},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.60.R3381}
}


@article{polo2019oscillations,
  title = {Oscillations and Decay of Superfluid Currents in a One-Dimensional Bose Gas on a Ring},
  author = {Polo, Juan and Dubessy, Romain and Pedri, Paolo and Perrin, H\'el\`ene and Minguzzi, Anna},
  journal = {Phys. Rev. Lett.},
  volume = {123},
  issue = {19},
  pages = {195301},
  numpages = {6},
  year = {2019},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.123.195301}
}


@misc{HL,
note = {For a uniform BEC, the size of the core of the vortex is the order of the healing length $\xi = (8 \pi na_m)^{-1/2}$, where $n$ is the density of the system and $a_m$ is twice of atomic scattering length, $a_m = 2a$ \cite{Tempere05}. Also the ratio between $\xi$ and the radius $r$ of the condensate takes the form of $\xi/R =(a_{ho}/R)^2$ \cite{Baym96}}}


@article{Ketterle_cooling,
title = {Evaporative Cooling of Trapped Atoms},
editor = {B. Bederson and H. Walther},
journal = {Advances In Atomic, Molecular, and Optical Physics},
publisher = {Academic Press},
volume = {37},
pages = {181-236},
year = {1996},
issn = {1049-250X},
doi = {https://doi.org/10.1016/S1049-250X(08)60101-9},
author = {W. Ketterle and N.J. Van Druten}
}

@article {Anderson198,
	author = {Anderson, M. H. and Ensher, J. R. and Matthews, M. R. and Wieman, C. E. and Cornell, E. A.},
	title = {Observation of Bose-Einstein Condensation in a Dilute Atomic Vapor},
	volume = {269},
	number = {5221},
	pages = {198--201},
	year = {1995},
	doi = {10.1126/science.269.5221.198},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	journal = {Science}
}

@article{Barrett01,
  title = {All-Optical Formation of an Atomic Bose-Einstein Condensate},
  author = {Barrett, M. D. and Sauer, J. A. and Chapman, M. S.},
  journal = {Phys. Rev. Lett.},
  volume = {87},
  issue = {1},
  pages = {010404},
  numpages = {4},
  year = {2001},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.87.010404}
}

@article{Nobel_Lec_Phillips,
  title = {Nobel Lecture: Laser cooling and trapping of neutral atoms},
  author = {Phillips, William D.},
  journal = {Rev. Mod. Phys.},
  volume = {70},
  issue = {3},
  pages = {721--741},
  numpages = {0},
  year = {1998},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.70.721}
}

@article{Tsatsos_turbulence,
title = {Quantum turbulence in trapped atomic Bose–Einstein condensates},
journal = {Physics Reports},
volume = {622},
pages = {1-52},
year = {2016},
issn = {0370-1573},
author = {Marios C. Tsatsos and Pedro E.S. Tavares and André Cidrim and Amilson R. Fritsch and Mônica A. Caracanhas and F. Ednilson A. {dos Santos} and Carlo F. Barenghi and Vanderlei S. Bagnato}}

@book{Wu_vorticity_07,
  title={Vorticity and vortex dynamics},
  author={Wu, Jie-Zhi and Ma, Hui-Yang and Zhou, M-D},
  year={2007},
  publisher={Springer Science \& Business Media}
}

@book{Saffman_vortex_95,
  title={Vortex dynamics},
  author={Saffman, Philip G},
  year={1995},
  publisher={Cambridge university press}
}

@book{Paoletti_QTurbulence_11,
  title={Quantum Turbulence},
  author={M. Paoletti and D. Lathrop},
  year={2011}
}

@article{Tsubota_QTurbulence_08,
  title={Quantum turbulence},
  author={Tsubota, Makoto},
  journal={Journal of the Physical Society of Japan},
  volume={77},
  number={11},
  pages={111006--111006},
  year={2008},
  publisher={The Physical Society of Japan}
}

@article{Kobayashi_QTurbulenc_07,
  title={Quantum turbulence in a trapped Bose-Einstein condensate},
  author={Kobayashi, Michikazu and Tsubota, Makoto},
  journal={Physical Review A},
  volume={76},
  number={4},
  pages={045603},
  year={2007},
  publisher={APS}
}

@article{White_vortices_14,
  title={Vortices and turbulence in trapped atomic condensates},
  author={White, Angela C and Anderson, Brian P and Bagnato, Vanderlei S},
  journal={Proceedings of the National Academy of Sciences},
  volume={111},
  number={Supplement 1},
  pages={4719--4726},
  year={2014},
  publisher={National Acad Sciences}
}

@article{Hodby2001,
  title = {Vortex Nucleation in Bose-Einstein Condensates in an Oblate, Purely Magnetic Potential},
  author = {Hodby, E. and Hechenblaikner, G. and Hopkins, S. A. and Marag\`o, O. M. and Foot, C. J.},
  journal = {Phys. Rev. Lett.},
  volume = {88},
  issue = {1},
  pages = {010405},
  numpages = {4},
  year = {2001},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.88.010405}
}

@article{Herve_ring:21,
	doi = {10.1088/1361-6455/ac0579},
	year = 2021,
	month = {jun},
	publisher = {{IOP} Publishing},
	journal={Journal of Physics B: Atomic, Molecular and Optical Physics},
	volume = {54},
	number = {12},
	pages = {125302},
	author = {M. de Goër de Herve and Y. Guo and C. De Rossi and A. Kumar and T. Badr and R. Dubessy and L. Longchambon and H. Perrin},
	title = {A versatile ring trap for quantum gases}
}

@article{Navez:16,
author = {Navez, Patrick and Pandey, Saurabh and Mas, Hector and Poulios, Konstantinos and Fernholz, T. and Von Klitzing, Wolf},
year = {2016},
month = {05},
pages = {},
title = {Matter-wave interferometers using TAAP rings},
volume = {18},
journal = {New Journal of Physics}
}

@article{Heathcote:08,
	doi = {10.1088/1367-2630/10/4/043012},
	year = 2008,
	month = {apr},
	journal={New Journal of Physics},
	publisher = {{IOP} Publishing},
	volume = {10},
	number = {4},
	pages = {043012},
	author = {W. H. Heathcote and E. Nugent and B. T. Sheard and C. J. Foot},
	title = {A ring trap for ultracold atoms in an {RF}-dressed state}
}

@article{Vortex_Madison,
  title = {Vortex Formation in a Stirred Bose-Einstein Condensate},
  author = {Madison, K. W. and Chevy, F. and Wohlleben, W. and Dalibard, J.},
  journal = {Phys. Rev. Lett.},
  volume = {84},
  issue = {5},
  pages = {806--809},
  numpages = {0},
  year = {2000},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.84.806}
}

@article{Feder_Nucleation,
  title={Nucleation of vortex arrays in rotating anisotropic Bose-Einstein condensates},
  author={Feder, David L and Clark, Charles W and Schneider, Barry I},
  journal={Physical Review A},
  volume={61},
  number={1},
  pages={011601},
  year={1999},
  publisher={APS}
}

@article{Aftalion_Vortices_2001,
  title={Vortices in a rotating Bose-Einstein condensate: Critical angular velocities and energy diagrams in the Thomas-Fermi regime},
  author={Aftalion, Amandine and Du, Qiang},
  journal={Physical Review A},
  volume={64},
  number={6},
  pages={063603},
  year={2001},
  publisher={APS}
}

@article{Tsubota_vortex_2002,
  title = {Vortex lattice formation in a rotating Bose-Einstein condensate},
  author = {Tsubota, M. and Kasamatsu, K. and Ueda, M.},
  journal = {Phys. Rev. A},
  volume = {65},
  issue = {2},
  pages = {023603},
  numpages = {4},
  year = {2002},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.65.023603}
}

@article{Fetter2009rotating,
  title={Rotating trapped bose-einstein condensates},
  author={Fetter, A. L.},
  journal={Reviews of Modern Physics},
  volume={81},
  number={2},
  pages={647},
  year={2009},
  publisher={APS}
}

@article{Engels2002,
  title={Nonequilibrium effects of anisotropic compression applied to vortex lattices in Bose-Einstein condensates},
  author={Engels, Peter and Coddington, Ian and Haljan, PC and Cornell, Eric A},
  journal={Physical review letters},
  volume={89},
  number={10},
  pages={100403},
  year={2002},
  publisher={APS}
}

@article{Madison_Stationary,
  title = {Stationary States of a Rotating Bose-Einstein Condensate: Routes to Vortex Nucleation},
  author = {Madison, K. W. and Chevy, F. and Bretin, V. and Dalibard, J.},
  journal = {Phys. Rev. Lett.},
  volume = {86},
  issue = {20},
  pages = {4443-4446},
  numpages = {0},
  year = {2001},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.86.4443}
}

@article {Vortex_Abo-Shaeer,
	author = {Abo-Shaeer, J. R. and Raman, C. and Vogels, J. M. and Ketterle, W.},
	title = {Observation of Vortex Lattices in Bose-Einstein Condensates},
	volume = {292},
	number = {5516},
	pages = {476-479},
	year = {2001},
	doi = {10.1126/science.1060182},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	journal = {Science}
}

@article{Price_2016,
	doi = {10.1088/1367-2630/18/11/113009},
	year = 2016,
	month = {nov},
	publisher = {{IOP} Publishing},
	volume = {18},
	number = {11},
	pages = {113009},
	author = {R M Price and D Trypogeorgos and D L Campbell and A Putra and A Vald{\'{e}}s-Curiel and I B Spielman},
	title = {Vortex nucleation in a Bose{\textendash}Einstein condensate: from the inside out},
	journal = {New Journal of Physics}
}

@book{Book_pethick:08,
  title={Bose-Einstein condensation in dilute gases},
  author={Pethick, Christopher J and Smith, Henrik},
  year={2008},
  publisher={Cambridge university press}
}


@article{Mcendoo_09,
  title={Small numbers of vortices in anisotropic traps},
  author={McEndoo, Suzanne and Busch, Th},
  journal={Physical Review A},
  volume={79},
  number={5},
  pages={053616},
  year={2009},
  publisher={APS}
}

@article{Williams_99,
  title={Preparing topological states of a Bose--Einstein condensate},
  author={Williams, J. E. and Holland, M. J.},
  journal={Nature},
  volume={401},
  number={6753},
  pages={568--572},
  year={1999},
  publisher={Nature Publishing Group}
}

@article{LoGullo:11,
  title = {{Structural change of vortex patterns in anisotropic Bose-Einstein condensates}},
  author = {Lo Gullo, N. and Busch, {\relax Th}. and Paternostro, M.},
  journal = {Phys. Rev. A},
  volume = {83},
  issue = {5},
  pages = {053612},
  numpages = {5},
  year = {2011},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.83.053612}
}


@article{Ring_Bell,
	doi = {10.1088/1367-2630/18/3/035003},
	year = 2016,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {18},
	number = {3},
	pages = {035003},
	author = {Thomas A Bell and Jake A P Glidden and Leif Humbert and Michael W J Bromley and Simon A Haine and Matthew J Davis and Tyler W Neely and Mark A Baker and Halina Rubinsztein-Dunlop},
	title = {Bose{\textendash}Einstein condensation in large time-averaged optical ring potentials},
	journal = {New Journal of Physics}
}

@article{Bell_2016,
	doi = {10.1088/1367-2630/18/3/035003},
	year = 2016,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {18},
	number = {3},
	pages = {035003},
	author = {Thomas A Bell and Jake A P Glidden and Leif Humbert and Michael W J Bromley and Simon A Haine and Matthew J Davis and Tyler W Neely and Mark A Baker and Halina Rubinsztein-Dunlop},
	title = {Bose{\textendash}Einstein condensation in large time-averaged optical ring potentials},
	journal = {New Journal of Physics}
}

@article{Bell_ring_16,
  title={Bose--Einstein condensation in large time-averaged optical ring potentials},
  author={Bell, Thomas A and Glidden, Jake AP and Humbert, Leif and Bromley, Michael WJ and Haine, Simon A and Davis, Matthew J and Neely, Tyler W and Baker, Mark A and Rubinsztein-Duavezlop, Halina},
  journal={New journal of Physics},
  volume={18},
  number={3},
  pages={035003},
  year={2016},
  publisher={IOP Publishing}
}

@book{Morandi_Low_D,
title = {Field Theories for Low-Dimensional Condensed Matter Systems},
series = {Springer Series in Solid-State Sciences},
publisher = {Springer, New York},
volume = {131},
year = {2000},
issn = {0171-1873},
author = {G. Morandi, P. Sodano, A. Tagliacozzo and V. Tognetti}
}
%https://www.springer.com/gp/book/9783540671770

%ring up
@article{QM_Lewenstein,
author = { Maciej   Lewenstein  and  Anna   Sanpera  and  Veronica   Ahufinger  and  Bogdan   Damski  and  Aditi   Sen(De)  and  Ujjwal   Sen },
title = {Ultracold atomic gases in optical lattices: mimicking condensed matter physics and beyond},
journal = {Advances in Physics},
volume = {56},
number = {2},
pages = {243-379},
year  = {2007},
publisher = {Taylor & Francis},
doi = {10.1080/00018730701223200}
}

@article{Qsim_Bloch,
  title={Quantum simulations with ultracold quantum gases},
  author={Bloch, Immanuel and Dalibard, Jean and Nascimbene, Sylvain},
  journal={Nature Physics},
  volume={8},
  number={4},
  pages={267--276},
  year={2012},
  publisher={Nature Publishing Group}
}

@article{QM_Bloch,
  title = {Many-body physics with ultracold gases},
  author = {Bloch, Immanuel and Dalibard, Jean and Zwerger, Wilhelm},
  journal = {Rev. Mod. Phys.},
  volume = {80},
  issue = {3},
  pages = {885--964},
  numpages = {0},
  year = {2008},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.80.885}
  }

@article{rev_Cohen,
  title = {Nobel Lecture: Manipulating atoms with photons},
  author = {Cohen-Tannoudji, Claude N.},
  journal = {Rev. Mod. Phys.},
  volume = {70},
  issue = {3},
  pages = {707--719},
  numpages = {0},
  year = {1998},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.70.707}
}

@article{BEC_Anderson,
	author = {Anderson, M. H. and Ensher, J. R. and Matthews, M. R. and Wieman, C. E. and Cornell, E. A.},
	title = {Observation of Bose-Einstein Condensation in a Dilute Atomic Vapor},
	volume = {269},
	number = {5221},
	pages = {198--201},
	year = {1995},
	doi = {10.1126/science.269.5221.198},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	journal = {Science}
}


@article{BEC_Davis,
  title = {Bose-Einstein Condensation in a Gas of Sodium Atoms},
  author = {Davis, K. B. and Mewes, M. -O. and Andrews, M. R. and van Druten, N. J. and Durfee, D. S. and Kurn, D. M. and Ketterle, W.},
  journal = {Phys. Rev. Lett.},
  volume = {75},
  issue = {22},
  pages = {3969--3973},
  numpages = {0},
  year = {1995},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.75.3969}
}

@article{BEC_Anglin,
  title={Bose--Einstein condensation of atomic gases},
  author={Anglin, James R and Ketterle, Wolfgang},
  journal={Nature},
  volume={416},
  number={6877},
  pages={211--218},
  year={2002},
  publisher={Nature Publishing Group}
}

@article{Optical_lattice_Becker,
	doi = {10.1088/1367-2630/12/6/065025},
	year = 2010,
	month = {jun},
	publisher = {{IOP} Publishing},
	volume = {12},
	number = {6},
	pages = {065025},
	author = {C Becker and P Soltan-Panahi and J Kronj{\"a}ger and S D{\"o}rscher and K Bongs and K Sengstock},
	title = {Ultracold quantum gases in triangular optical lattices},
	journal = {New Journal of Physics}
}

@article{Optical_lattice_Petsas,
  title = {Crystallography of optical lattices},
  author = {Petsas, K. I. and Coates, A. B. and Grynberg, G.},
  journal = {Phys. Rev. A},
  volume = {50},
  issue = {6},
  pages = {5173--5189},
  numpages = {0},
  year = {1994},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.50.5173}
}

@article{Optical_lattice_Grynberg,
  title={Quantized motion of cold cesium atoms in two-and three-dimensional optical potentials},
  author={Grynberg, G and Lounis, B and Verkerk, P and Courtois, J-Y and Salomon, C},
  journal={Physical review letters},
  volume={70},
  number={15},
  pages={2249},
  year={1993},
  publisher={APS}
}

@article{Painted_Henderson,
	doi = {10.1088/1367-2630/11/4/043030},
	year = 2009,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {11},
	number = {4},
	pages = {043030},
	author = {K Henderson and C Ryu and C MacCormick and M G Boshier},
	title = {Experimental demonstration of painting arbitrary and dynamic potentials for Bose{\textendash}Einstein condensates},
	journal = {New Journal of Physics}
}

@article{Llorente_19,
  title = {Expanding ring-shaped Bose-Einstein condensates as analogs of cosmological models: Analytical characterization of the inflationary dynamics},
  author = {Gomez Llorente, J. M. and Plata, J.},
  journal = {Phys. Rev. A},
  volume = {100},
  issue = {4},
  pages = {043613},
  numpages = {13},
  year = {2019},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.100.043613}
}

@article{Bloch_Mendez,
  title={Wannier{\textendash}Stark ladders and Bloch oscillations in superlattices},
  author={Mendez, Emilio E and Bastard, G{\'e}rald},
  journal={Physics Today},
  volume={46},
  pages={34--34},
  year={1993},
  publisher={American Institute of Physics}
}

@article{Toroidal__Wright,
  title = {Toroidal optical dipole traps for atomic Bose-Einstein condensates using Laguerre-Gaussian beams},
  author = {Wright, E. M. and Arlt, J. and Dholakia, K.},
  journal = {Phys. Rev. A},
  volume = {63},
  issue = {1},
  pages = {013608},
  numpages = {7},
  year = {2000},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.63.013608}
}

@article{Adiabatic__Wright,
  title = {Time{\textendash}Averaged Adiabatic Potentials: Versatile Matter-Wave Guides and Atom Traps},
  author = {Lesanovsky, Igor and von Klitzing, Wolf},
  journal = {Phys. Rev. Lett.},
  volume = {99},
  issue = {8},
  pages = {083001},
  numpages = {4},
  year = {2007},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.99.083001}
}

@article{Gupta05,
  title = {Bose-Einstein Condensation in a Circular Waveguide},
  author = {Gupta, S. and Murch, K. W. and Moore, K. L. and Purdy, T. P. and Stamper-Kurn, D. M.},
  journal = {Phys. Rev. Lett.},
  volume = {95},
  issue = {14},
  pages = {143201},
  numpages = {4},
  year = {2005},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.95.143201}
}

@article{Arnold_06,
  title = {Large magnetic storage ring for Bose-Einstein condensates},
  author = {Arnold, A. S. and Garvie, C. S. and Riis, E.},
  journal = {Phys. Rev. A},
  volume = {73},
  issue = {4},
  pages = {041606},
  numpages = {4},
  year = {2006},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.73.041606}
}


@article{Bloch_Dum,
  title={Gauge structures in atom-laser interaction: Bloch oscillations in a dark lattice},
  author={Dum, R and Olshanii, M},
  journal={Physical review letters},
  volume={76},
  number={11},
  pages={1788},
  year={1996},
  publisher={APS}
}

@article{Angularmomentum_Andersen,
  title = {Quantized Rotation of Atoms from Photons with Orbital Angular Momentum},
  author = {Andersen, M. F. and Ryu, C. and Clad\'e, Pierre and Natarajan, Vasant and Vaziri, A. and Helmerson, K. and Phillips, W. D.},
  journal = {Phys. Rev. Lett.},
  volume = {97},
  issue = {17},
  pages = {170406},
  numpages = {4},
  year = {2006},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.97.170406}
}

@article{ring_angela,
  title = {Odd-petal-number states and persistent flows in spin-orbit-coupled Bose-Einstein condensates},
  author = {White, Angela C. and Zhang, Yongping and Busch, Thomas},
  journal = {Phys. Rev. A},
  volume = {95},
  issue = {4},
  pages = {041604},
  numpages = {6},
  year = {2017},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.95.041604}
}

@article{TCBEC_Modugno,
  title = {Two Atomic Species Superfluid},
  author = {Modugno, G. and Modugno, M. and Riboli, F. and Roati, G. and Inguscio, M.},
  journal = {Phys. Rev. Lett.},
  volume = {89},
  issue = {19},
  pages = {190404},
  numpages = {4},
  year = {2002},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.89.190404}
}


@article{TCBEC_McCarron,
  title = {Dual-species Bose-Einstein condensate of $^{87}\mathrm{Rb}$ and $^{133}\mathrm{Cs}$},
  author = {McCarron, D. J. and Cho, H. W. and Jenkin, D. L. and K\"oppinger, M. P. and Cornish, S. L.},
  journal = {Phys. Rev. A},
  volume = {84},
  issue = {1},
  pages = {011603},
  numpages = {4},
  year = {2011},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.84.011603}
}

@article{BEC_Trippenbach,
	doi = {10.1088/0953-4075/33/19/314},
	year = 2000,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {33},
	number = {19},
	pages = {4017--4031},
	author = {Marek Trippenbach and Krzysztof G{\'{o}}ral and Kazimierz Rzazewski and Boris Malomed and Y B Band},
	title = {Structure of binary Bose-Einstein condensates},
	journal = {Journal of Physics B: Atomic, Molecular and Optical Physics}
}

@article{Feshbach_Resonance_light_Fedichev,
  title = {Influence of Nearly Resonant Light on the Scattering Length in Low-Temperature Atomic Gases},
  author = {Fedichev, P. O. and Kagan, Yu. and Shlyapnikov, G. V. and Walraven, J. T. M.},
  journal = {Phys. Rev. Lett.},
  volume = {77},
  issue = {14},
  pages = {2913--2916},
  numpages = {0},
  year = {1996},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.77.2913}
}

@article{Instability_Tojo,
  title = {Controlling phase separation of binary Bose-Einstein condensates via mixed-spin-channel Feshbach resonance},
  author = {Tojo, Satoshi and Taguchi, Yoshihisa and Masuyama, Yuta and Hayashi, Taro and Saito, Hiroki and Hirano, Takuya},
  journal = {Phys. Rev. A},
  volume = {82},
  issue = {3},
  pages = {033609},
  numpages = {5},
  year = {2010},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.82.033609}
}

@article{Feshbach_Resonance_Courteille,
  title = {Observation of a Feshbach Resonance in Cold Atom Scattering},
  author = {Courteille, Ph. and Freeland, R. S. and Heinzen, D. J. and van Abeelen, F. A. and Verhaar, B. J.},
  journal = {Phys. Rev. Lett.},
  volume = {81},
  issue = {1},
  pages = {69--72},
  numpages = {0},
  year = {1998},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.81.69}
}

@article{Vortex_Matthews,
  title = {Vortices in a Bose-Einstein Condensate},
  author = {Matthews, M. R. and Anderson, B. P. and Haljan, P. C. and Hall, D. S. and Wieman, C. E. and Cornell, E. A.},
  journal = {Phys. Rev. Lett.},
  volume = {83},
  issue = {13},
  pages = {2498--2501},
  numpages = {0},
  year = {1999},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.83.2498}
}

@article{Vortex_Bretin,
  title = {Fast Rotation of a Bose-Einstein Condensate},
  author = {Bretin, Vincent and Stock, Sabine and Seurin, Yannick and Dalibard, Jean},
  journal = {Phys. Rev. Lett.},
  volume = {92},
  issue = {5},
  pages = {050403},
  numpages = {4},
  year = {2004},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.92.050403}
}

@book{Feynman_vortex,
title = {Chapter II Application of Quantum Mechanics to Liquid Helium},
editor = {C.J. Gorter},
series = {Progress in Low Temperature Physics},
publisher = {Elsevier},
volume = {1},
pages = {17 - 53},
year = {1955},
issn = {0079-6417},
author = {R.P. Feynman}
}

@article{Artificial_gauge_Courteille,
  title = {Colloquium: Artificial gauge potentials for neutral atoms},
  author = {Dalibard, Jean and Gerbier, Fabrice and Juzeli\ifmmode \bar{u}\else \={u}\fi{}nas, Gediminas and \"Ohberg, Patrik},
  journal = {Rev. Mod. Phys.},
  volume = {83},
  issue = {4},
  pages = {1523--1543},
  numpages = {0},
  year = {2011},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.83.1523}
}

@article{Mochol_mag,
  title={Artificial magnetic field induced by an evanescent wave},
  author={Mochol, Ma{\l}gorzata and Sacha, Krzysztof},
  journal={Scientific reports},
  volume={5},
  pages={7672},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{Controlling_phase_Wen,
  title = {Controlling phase separation of a two-component Bose{\textendash}Einstein condensate by confinement},
  author = {Wen, L. and Liu, W. M. and Cai, Yongyong and Zhang, J. M. and Hu, Jiangping},
  journal = {Phys. Rev. A},
  volume = {85},
  issue = {4},
  pages = {043602},
  numpages = {8},
  year = {2012},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.85.043602}
}

@article{Controlling_phase_Papp,
  title = {Tunable Miscibility in a Dual-Species Bose-Einstein Condensate},
  author = {Papp, S. B. and Pino, J. M. and Wieman, C. E.},
  journal = {Phys. Rev. Lett.},
  volume = {101},
  issue = {4},
  pages = {040402},
  numpages = {4},
  year = {2008},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.101.040402}}
}

@article{Controlling_phase_Thalhammer,
  title = {Double Species Bose-Einstein Condensate with Tunable Interspecies Interactions},
  author = {Thalhammer, G. and Barontini, G. and De Sarlo, L. and Catani, J. and Minardi, F. and Inguscio, M.},
  journal = {Phys. Rev. Lett.},
  volume = {100},
  issue = {21},
  pages = {210402},
  numpages = {4},
  year = {2008},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.100.210402}
}

@article{Controlling_phase_Merhasin,
	doi = {10.1088/0953-4075/38/7/009},
	year = 2005,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {38},
	number = {7},
	pages = {877--892},
	author = {Ilya M Merhasin and Boris A Malomed and Rodislav Driben},
	title = {Transition to miscibility in a binary Bose{\textendash}Einstein condensate induced by linear coupling},
	journal = {Journal of Physics B: Atomic, Molecular and Optical Physics}
}


@article{wright2013driving,
  title = {Driving Phase Slips in a Superfluid Atom Circuit with a Rotating Weak Link},
  author = {Wright, K. C. and Blakestad, R. B. and Lobb, C. J. and Phillips, W. D. and Campbell, G. K.},
  journal = {Phys. Rev. Lett.},
  volume = {110},
  issue = {2},
  pages = {025302},
  numpages = {5},
  year = {2013},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.110.025302}
}


@article{gauge_field_Goldman,
	doi = {10.1088/0034-4885/77/12/126401},
	year = 2014,
	month = {nov},
	publisher = {{IOP} Publishing},
	volume = {77},
	number = {12},
	pages = {126401},
	author = {N Goldman and G Juzeli{\={u}}nas and P Öhberg and I B Spielman},
	title = {Light-induced gauge fields for ultracold atoms},
	journal = {Reports on Progress in Physics}
}

@article{CHEN20152193,
  title={Vortices in a Rotating Spin-Orbit-Coupled Bose—Einstein Condensate under Extreme Elongation in a Harmonic Plus Quartic Trap},
  author={Chen, Guang-Ping and Chen, Si-Lin and Xie, Zheng-Wei and Zhang, Xiao-Fei and Zhang, Shou-Gang},
  journal={Communications in Theoretical Physics},
  volume={66},
  number={1},
  pages={53},
  year={2016},
  publisher={IOP Publishing}
}

@article{Rashi_fiber_evan,
  title = {Creating superfluid vortex rings in artificial magnetic fields},
  author = {Sachdeva, Rashi and Busch, Thomas},
  journal = {Phys. Rev. A},
  volume = {95},
  issue = {3},
  pages = {033615},
  numpages = {8},
  year = {2017},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.95.033615}
}

@article{Williams_02,
  title = {Dynamical Instability of a Condensate Induced by a Rotating Thermal Gas},
  author = {Williams, J. E. and Zaremba, E. and Jackson, B. and Nikuni, T. and Griffin, A.},
  journal = {Phys. Rev. Lett.},
  volume = {88},
  issue = {7},
  pages = {070401},
  numpages = {4},
  year = {2002},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.88.070401}
}


@article{Bai_double_well,
title = {Condensates in double-well potential with synthetic gauge potentials and vortex seeding},
journal = {Physics Letters A},
volume = {382},
number = {34},
pages = {2376 - 2381},
year = {2018},
issn = {0375-9601},
author = {Rukmani Bai and Arko Roy and D. Angom and P. Muruganandam}
}

@article{Henderson_ring_2009,
	doi = {10.1088/1367-2630/11/4/043030},
	year = 2009,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {11},
	number = {4},
	pages = {043030},
	author = {K Henderson and C Ryu and C MacCormick and M G Boshier},
	title = {Experimental demonstration of painting arbitrary and dynamic potentials for Bose{\textendash}Einstein condensates},
	journal = {New Journal of Physics}
}


@article{Ring_Amico,
  title = {Quantum Many Particle Systems in Ring-Shaped Optical Lattices},
  author = {Amico, Luigi and Osterloh, Andreas and Cataliotti, Francesco},
  journal = {Phys. Rev. Lett.},
  volume = {95},
  issue = {6},
  pages = {063201},
  numpages = {4},
  year = {2005},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.95.063201}
}

@article{Heathcote_ring_2008,
	doi = {10.1088/1367-2630/10/4/043012},
	year = 2008,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {10},
	number = {4},
	pages = {043012},
	author = {W H Heathcote and E Nugent and B T Sheard and C J Foot},
	title = {A ring trap for ultracold atoms in an {RF}-dressed state},
	journal = {New Journal of Physics}
}

@article{Eckern_ring_2002,
  title={Persistent currents versus phase breaking in mesoscopic metallic samples},
  author={Eckern, Ulrich and Schwab, Peter},
  journal={Journal of low temperature physics},
  volume={126},
  number={3},
  pages={1291--1304},
  year={2002},
  publisher={Springer}
}

@article{Ferris_wheel_Lemb,
author = {V. E. Lembessis and A. Alqarni and S. Alshamari and A. Siddig and O. M. Aldossary},
journal = {J. Opt. Soc. Am. B},
number = {6},
pages = {1122--1129},
publisher = {OSA},
title = {Artificial gauge magnetic and electric fields for free two-level atoms interacting with optical Ferris wheel light fields},
volume = {34},
month = {Jun},
year = {2017},
doi = {10.1364/JOSAB.34.001122}
}

@article{Bao_dim,
title = {Numerical solution of the Gross–Pitaevskii equation for Bose–Einstein condensation},
journal = {Journal of Computational Physics},
volume = {187},
number = {1},
pages = {318 - 342},
year = {2003},
issn = {0021-9991},
doi = {https://doi.org/10.1016/S0021-9991(03)00102-5},
author = {Weizhu Bao and Dieter Jaksch and Peter A. Markowich}
}

@article{Fleck_fft,
  title={Time-dependent propagation of high energy laser beams through the atmosphere},
  author={Fleck, JA and Morris, JR and Feit, MD},
  journal={Applied physics},
  volume={10},
  number={2},
  pages={129--160},
  year={1976},
  publisher={Springer}
}

@article{Feit_fft,
  title={Solution of the Schr{\"o}dinger equation by a spectral method},
  author={Feit, MD and Fleck Jr, JA and Steiger, A},
  journal={Journal of Computational Physics},
  volume={47},
  number={3},
  pages={412--433},
  year={1982},
  publisher={Academic Press}
}

@article{Wenvortex,
  title={Formation and structure of vortex lattices in a rotating double-well Bose-Einstein condensate},
  author={Wen, LH and Luo, XB},
  journal={Laser Physics Letters},
  volume={9},
  number={8},
  pages={618},
  year={2012},
  publisher={IOP Publishing}
}

@article{Vortex_McEndoo_Busch,
  title = {Small numbers of vortices in anisotropic traps},
  author = {McEndoo, S. and Busch, Th.},
  journal = {Phys. Rev. A},
  volume = {79},
  issue = {5},
  pages = {053616},
  numpages = {7},
  year = {2009},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.79.053616}
}

@article{Vortex_Gullo_Busch,
  title = {Structural change of vortex patterns in anisotropic Bose-Einstein condensates},
  author = {Lo Gullo, N. and Busch, Th. and Paternostro, M.},
  journal = {Phys. Rev. A},
  volume = {83},
  issue = {5},
  pages = {053612},
  numpages = {5},
  year = {2011},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.83.053612}
}

@article{Bradley2008,
  title={Bose-Einstein condensation from a rotating thermal cloud: Vortex nucleation and lattice formation},
  author={Bradley, AS and Gardiner, CW and Davis, MJ},
  journal={Physical Review A},
  volume={77},
  number={3},
  pages={033616},
  year={2008},
  publisher={APS}
}

@article{Abrikosov1957,
  title={On the magnetic properties of superconductors of the second group},
  author={Abrikosov, Alexei A},
  journal={Sov. Phys. JETP},
  volume={5},
  pages={1174--1182},
  year={1957}
}

@article{ORiordan2016,
  title = {Moir\'e superlattice structures in kicked Bose-Einstein condensates},
  author = {O'Riordan, L. J. and White, A. C. and Busch, Th.},
  journal = {Phys. Rev. A},
  volume = {93},
  issue = {2},
  pages = {023609},
  numpages = {6},
  year = {2016},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.93.023609}
}

@article{Baym96,
  title = {Ground-State Properties of Magnetically Trapped Bose-Condensed Rubidium Gas},
  author = {Baym, Gordon and Pethick, C. J.},
  journal = {Phys. Rev. Lett.},
  volume = {76},
  issue = {1},
  pages = {6--9},
  numpages = {0},
  year = {1996},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.76.6}
}

@article{Tempere05,
  title = {Path-integral mean-field description of the vortex state in the BEC-to-BCS crossover},
  author = {Tempere, J. and Wouters, M. and Devreese, J. T.},
  journal = {Phys. Rev. A},
  volume = {71},
  issue = {3},
  pages = {033631},
  numpages = {4},
  year = {2005},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.71.033631}
}

@book{Pitaevskii2016,
  title={Bose-Einstein condensation and superfluidity},
  author={Pitaevskii, Lev and Stringari, Sandro},
  volume={164},
  year={2016},
  publisher={Oxford University Press}
}

@article{Bland2020,
  title={Persistent current formation in double-ring geometries},
  author={Bland, Thomas and Marolleau, Quentin and Comaron, Paolo and Malomed, BA and Proukakis, NP},
  journal={Journal of Physics B: Atomic, Molecular and Optical Physics},
  volume={53},
  number={11},
  pages={115301},
  year={2020},
  publisher={IOP Publishing}
}

@article{1D_Helm:15,
  title = {Sagnac Interferometry Using Bright Matter-Wave Solitons},
  author = {Helm, J. L. and Cornish, S. L. and Gardiner, S. A.},
  journal = {Phys. Rev. Lett.},
  volume = {114},
  issue = {13},
  pages = {134101},
  numpages = {5},
  year = {2015},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.114.134101}
}

